Anomalous topological waves in strongly amorphous scattering networks

Topological insulators are crystalline materials that have revolutionized our ability to control wave transport. They provide us with unidirectional channels that are immune to obstacles, defects or local disorder, and can even survive some random deformations of their crystalline structures. However, they always break down when the level of disorder or amorphism gets too large, transitioning to a topologically trivial Anderson insulating phase. Here, we demonstrate a two-dimensional amorphous topological regime that survives arbitrarily strong levels of amorphism. We implement it for electromagnetic waves in a non-reciprocal scattering network and experimentally demonstrate the existence of unidirectional edge transport in the strong amorphous limit. This edge transport is shown to be mediated by an anomalous edge state whose topological origin is evidenced by direct topological invariant measurements. Our findings extend the reach of topological physics to a new class of systems in which strong amorphism can induce, enhance and guarantee the topological edge transport instead of impeding it.

==> Results.tex <==
Remark : The plateaus of the QHE are better resolved when disorder is added. 

==> title_discussion.tex <==
Current selection:

Anomalous topological waves in strongly amorphous scattering networks

Anomalous topology in strongly amorphous microwave scattering networks

keyword noun: 
1st class Topology/ical;  strongly amorphous;  anomalous network
2nd calss: scattering; wave; nonreciprocal/unidirectional;  transport

Main messages:
1 Amorphous non-reciprocal networks can exhibit anomalous topology, resisting trivial transition, coexisting with any level of spatial disorder, ultimately enhanced by the strong amorphism. 
2 We calculate and directly measure the topological index confirming the non-trivial topology in strong amorphous structure
3 We do this work back and forth between theory and experiment.


Some other titles:
10. 3. 2022
I Amorphous topological scattering network (broad but ...)
II. Anomalous topological waves in/surviving the strongly amorphous regime; (regime is risky although there are more weird titles...)
III. Unidirectional topological transport in strongly amorphous scattering networks;  (unidirectional transport as title may not attractive?)
IV. Strongly amorphous scattering networks with enhanced anomalous topology (....)
V.  Anomalous topological waves enhanced by strong amorphism 
(may be amorphous should be put as at least the same important as (anomalous) topology in title )

10. 4. 2022
I (shorter version) Anomalous topology in strongly amorphous (scattering) network
II ( try to cover all the main message) Unidirectional transport in strongly amorphous network: anomalous topology and direct measurement/ observation 
Or Anomalous topology in strongly amorphous network: unidirectional transport and direct measurement/ observation
III (Short version)Strong amorphism enhance anomalous topology
IV (more fancy hhhh) Matthew effect of topology in strong amorphous network (It may look more like a title for report of our research.)
from: "For to everyone who has will more be given, and he will have abundance; but for him who has not, even what he has will be taken away" — Matthew 25:29, RSV. to convey: Anomalous phase is enhance while Chern becomes trivial.


Story

The interplay between amorphism and topology has been left largely unexplored. Past works focused on the weakly amorphous regimes, and topology is lost at strong amorphism level. Largely amorphous systems are generally trivial insulators. In scattering networks, we have a chance to observe richer topological phenomena, a well-known example of which is the anomalous topological insulator, that has recently been demonstrated as being more resilient than the Chern. NEED TO DO A GOOD LITERATURE REVIEW ON AMORPHOUS TIS

Here we demonstrate a photonic anomalous topological phase that can survive arbitrarily large levels of amorphism, way beyond the weak amorphous regime. We construct such a phase from random oriented Eulerian graphs, which are then mapped onto physical amorphous non-reciprocal network of circulators. We experimentally validate the survival of the edge mode and proove its topological origin by direct measurements of the topological invairant, and we elucidate the physics.

Consider an oriented graph representing a scattering network (graph shown in Fig. 1a)...the edge mode is still there in the strong amorphous limit as we expected/intuited...

..and this is surprising, because if you do this with a Chern mode it does not work... (Fig.2) so this amorphous topological phase is topologically distinct from the amorphous Chern, which is a trivial insulator. To validate this experimentally, we built an interface...

...so what is going on? to elucidate the physics, we track the evolution of the BS from the clean limit to the strongly amorphous case by checking the transmission (edge and bulk). Describe the figure 3. we you increase alpha, you start in a band, not in a gap

...We still need to prove/shed light on the topological character of this amorphous phase/prove the nontrivial topology. We propose a measurement of the topological invariant, we measure it (describe Fig.4). So it really is topological.

Conclude.

-------

Disorder and amorphism generally break topological phases. While TIs have been demonstrated with strong resilience to disorder, resilience to strong amorphism is still elusive.


Fig. 1
